Mechanic: the MPI/HDF code framework for dynamical astronomy

We introduce the Mechanic, a new open-source code framework. It is designed to reduce the development effort of scientific applications by providing unified API (Application Programming Interface) for configuration, data storage and task management. The communication layer is based on the well-established Message Passing Interface (MPI) standard, which is widely used on variety of parallel computers and CPU-clusters. The data storage is performed within the Hierarchical Data Format (HDF5). The design of the code follows em core-module approach which allows to reduce the user's codebase and makes it portable for single- and multi-CPU environments. The framework may be used in a local user's environment, without administrative access to the cluster, under the PBS or Slurm job schedulers. It may become a helper tool for a wide range of astronomical applications, particularly focused on processing large data sets, such as dynamical studies of long-term orbital evolution of planetary systems with Monte Carlo methods, dynamical maps or evolutionary algorithms. It has been already applied in numerical experiments conducted for Kepler-11 (Migaszewski et al., 2012), and nuOctantis planetary systems (Go\'zdziewski et al., 2013). In this paper we describe the basics of the framework, including code listings for the implementation of a sample user's module. The code is illustrated on a model Hamiltonian introduced by (Froeschle et al., 2000) presenting the Arnold diffusion. The Arnold Web is shown with the help of the MEGNO (Mean Exponential Growth of Nearby Orbits) fast indicator (Go\'zdziewski et al., 2008a) applied onto symplectic SABA integrators family (Laskar and Robutel, 2001).

==> aweb_simple-c.tex <==
/*
	mpicc -fPIC -Dpic -shared aweb.c \
  	-o libmechanic_module_aweb.so \
  	-lmechanic -lm -lhdf5 

  mpirun -np 2048 mechanic -p aweb \
    --xres=2048 --yres=2048 \
    --xmin=-0.5 --xmax=1.5  \
    --ymin=-0.5 --ymax=1.5  \
    --step=0.5 --eps=0.04   \
    --task-checkpoints=5    \
    --name=arnold-web
 */

#include "mechanic.h"
#include <math.h>

#define MAX_SNAPSHOTS 10

int saba3(double *state, double step, 
    double tstart, double tend, double eps, 
    double *megno, double *err);

/* Implements Init() */
int Init(init *i) {
  i->banks_per_task = 2;
  return SUCCESS;
}

/* Implements Setup() */
int Setup(setup *s) {
  s->options[0] = (options) {
    .space = "aweb", .name = "step", .shortName = '\0',
    .value = '0.5', .type = C_DOUBLE,
    .description = "Integrator step size"
  };
  s->options[1] = (options) {
    .space = "aweb", .name = "eps", .shortName = '\0',
    .value = '0.01', .type = C_DOUBLE,
    .description = "The perturbation parameter"
  };
  s->options[2] = (options) OPTIONS_END;

  return SUCCESS;
}

/* Implements Storage() */
int Storage(pool *p) {
  int snapshots;

  // Security check
  MReadOption(p, "task-checkpoints", &snapshots);
  if (snapshots > MAX_SNAPSHOTS) {
    snapshots = MAX_SNAPSHOTS;
    MWriteOption(p, "task-checkpoints", &snapshots);
  }

  // Path: /Pools/pool-ID/Tasks/result
  p->task->storage[0].layout = (schema) {
    .name = "result",
    .rank = 4,
    .dims[0] = 1, //y-dim
    .dims[1] = 1, //x-dim
    .dims[2] = MAX_SNAPSHOTS,
    .dims[3] = 2,
    .use_hdf = HDF_NORMAL_STORAGE,
    .storage_type = STORAGE_TEXTURE,
    .datatype = H5T_NATIVE_DOUBLE
  };

  // Temporary storage for the state variables
  p->task->storage[1].layout = (schema) {
    .name = "state",
    .rank = 2,
    .dims[0] = 1,
    .dims[1] = 24,
    .use_hdf = HDF_TEMP_STORAGE,
    .storage_type = STORAGE_LIST,
    .datatype = H5T_NATIVE_DOUBLE
  };

  return SUCCESS;
}

/* Implements TaskPrepare() */
int TaskPrepare(pool *p, task *t) {
  double state[24];
  double r[1][1][MAX_SNAPSHOTS][2];
  double xmin, xmax, ymin, ymax;
  double stepx, stepy;
  int xres, yres, i;
  
  if (t->cid == 0) {
    MReadOption(p, "xmin", &xmin);
    MReadOption(p, "xmax", &xmax);
    MReadOption(p, "ymin", &ymin);
    MReadOption(p, "ymax", &ymax);

    MReadOption(p, "xres", &xres);
    MReadOption(p, "yres", &yres);

    stepx = (xmax-xmin)/((double)xres);
    stepy = (ymax-ymin)/((double)yres);

    // Initial data
    for (i = 0; i < 24; i++)
      state[i] = 0.0;

    state[3] = xmin + t->location[1]*stepx;
    state[4] = ymin + t->location[0]*stepy;
    state[5] = 1.0;

    // Randomize the tangent vector
    for (i = 6; i < 12; i++)
      state[i] = rand()/(RAND_MAX+1.0);

    MWriteData(t, "state", &state[0]);

    // Prepare the result buffer
    for (i = 0; i < MAX_SNAPSHOTS; i++) {
      r[0][0][i][0] = 0.0;
      r[0][0][i][1] = 0.0;
    }
    MWriteData(t, "result", &r[0][0][0][0]);
  }

  return SUCCESS;
}
  
/* Implements TaskProcess() */
int TaskProcess(pool *p, task *t) {
  double state[24];
  double result[1][1][MAX_SNAPSHOTS][2];
  double tstart = 0.0, tend = 0.0, step = 0.0;
  double megno = 0.0, err = 0.0, eps = 0.0;
  int snapshots, status = SUCCESS;

  MReadOption(p, "task-checkpoints", &snapshots);
  MReadOption(p, "eps", &eps);
  MReadOption(p, "step", &step);

  // power-based time intervals
  if (t->cid == 0) tstart = 0.0;
  else tstart = pow(10, t->cid + 4);
  
  tend = pow(10, t->cid + 5);

  step = step*(pow(5,0.5)-1)/2.0;

  MReadData(t, "state", &state[0]);

  if (t->cid > 0) {
    MReadData(t, "result", &result[0][0][0][0]);
  }

  // Numerical integration goes here
  status = saba3(state, step, tstart, tend, 
      eps, &megno, &err);
  if (status < 0) return MODULE_ERR_OTHER;
  
  // Assign the master result
  result[0][0][t->cid][0] = megno;
  result[0][0][t->cid][1] = err;

  MWriteData(t, "result", &result[0][0][0][0]);
  MWriteData(t, "state", &state[0]);

  if (t->cid + 1 == snapshots) return TASK_FINALIZE;
  return TASK_CHECKPOINT;
}

/* Implements Receive() */
int Receive(int mpi_size, int node, int sender, int tag, pool *p, void *buffer) {
  if (node == MASTER) {
    if (tag == TAG_RESULT) {
      if ((p->completed % 1000) == 0) {
        Message(MESSAGE_RESULT, "Completed %6d of %6d tasks\n", p->completed, p->pool_size);
      }
    }
  }
  return SUCCESS;
}

/**
 * Symplectic MEGNO (Gozdziewski, Breiter & Borczyk, MNRAS, 2008)
 * with the SABA3 integrator (Laskar & Robutel, CMDA, 2001)
 */
int saba3(double *state, double step,
  double tstart, double tend, double eps,
  double *megno, double *err) {
  return 0;
}


